Evolutional Deep Neural Network

The notion of an Evolutional Deep Neural Network (EDNN) is introduced for the solution of partial differential equations (PDE). The parameters of the network are trained to represent the initial state of the system only, and are subsequently updated dynamically, without any further training, to provide an accurate prediction of the evolution of the PDE system. In this framework, the network parameters are treated as functions with respect to the appropriate coordinate and are numerically updated using the governing equations. By marching the neural network weights in the parameter space, EDNN can predict state-space trajectories that are indefinitely long, which is difficult for other neural network approaches. Boundary conditions of the PDEs are treated as hard constraints, are embedded into the neural network, and are therefore exactly satisfied throughout the entire solution trajectory. Several applications including the heat equation, the advection equation, the Burgers equation, the Kuramoto Sivashinsky equation and the Navier-Stokes equations are solved to demonstrate the versatility and accuracy of EDNN. The application of EDNN to the incompressible Navier-Stokes equation embeds the divergence-free constraint into the network design so that the projection of the momentum equation to solenoidal space is implicitly achieved. The numerical results verify the accuracy of EDNN solutions relative to analytical and benchmark numerical solutions, both for the transient dynamics and statistics of the system.

==> Euler_backup <==
\subsubsection{1D Euler's equations}\label{Res:Euler's}
In this section we solve 1-D Euler's equations using ENN as an example of hyperbolic systems. The numerical treatment of hyperbolic conservation laws is challenging in the presents of shock waves. We solve the contact discontinuity  problems as a standard test cases for solutions of conservation laws. The 1-D Euler's equation is as follow: 
\be
\partial_t \boldsymbol{U} + \nabla \cdot F(\boldsymbol{U}) = 0
\ee
where $\boldsymbol{U}$ is the conserved state and $F(\cdot)$ is the flux, which are both defined as follow: 
\be
\boldsymbol{U} = \left(\begin{matrix}
           \rho \\
           \rho u \\
           \rho E
         \end{matrix}\right)
         , F(\boldsymbol{U}) = \left(\begin{matrix}
           \rho u \\
           \rho u^2 + p \\
           u(\rho E + p)
         \end{matrix}\right)
\ee
where $\rho$, $u$, $E$ and $p$ represent fluid density, velocity, total energy and pressure respectively. For a polytropic gas, the pressure can be related with velocity and energy by the state equation: 
\be
p = (\gamma - 1)\left(\rho E -\frac{1}{2}\rho u^2\right). 
\ee
The above equations form a closed system and the solution is uniquely determined with proper initial and boundary conditions. The following initial conditions are applied for the numerical solution of Euler's equation: 
\be
\rho(x, 0),u(x, 0),p(x, 0)=\left\{\begin{array}{ll}1.4,1.0,1.0, & x<0.5 \\ 1.0,1.0,1.0 & x>0.5\end{array} \right. x\in [0,1], 
\ee
Dirichlet boundary conditions are enforced at $x = \pm 1$ that are consistent with the initial condition. The analytical solution of this as follow: 
\be
\rho(x, t)=\left\{\begin{array}{ll}1.4, & x<t+0.5 \\ 1.0,& x>t+0.5\end{array} \right. , u(x,t) = 1.0,\, p(x,t)=1.0
\ee
The numerical solution of the contact discontinuity problem at $t = 0.1$ is shown in Fig. (\ref{1dEuler_sol}). The corresponding parameters of the neural network and discretization are shown in Tab. (\ref{1dEuler_params}). It can be observed that the solutions travel at the same speed as the analytical solution, but the quality of the solution is not satisfactory. There are oscillations at the two sides of shock wave solution, which are often observed in some traditional numerical schemes as well. Using $L^1$ penalty at the training of initial condition suppresses the oscillation around the shock wave (case 3e), but it will introduce diffusion and the solution does not remain vertical for the velocity and energy. In case (4e), the neural network size is increased with a weaker penalty on the weights at initial training. The solution quality is improved compared to other three cases, but the oscillation on velocity $u$ is still severe. The discretization of hyperbolic systems, especially Euler equation, using ENN still need to be investigated in a more systematic and detailed manner in a future work. 
\begin{center}\label{1dEuler_params}
\begin{tabular}{ ccccccccc } 
 \hline
 Case & $n_L$ & $L$ & $N_x$ & $\Delta t$  & $\sigma$ & $\lambda$\\ 
 \hline
 1e & $10$ & $4$ & $1000$ &  $1 \times 10^{-4}$ & $\mathrm{tanh}$ & $0$\\  
 2e & $10$ & $4$ & $1000$ &  $1 \times 10^{-4}$ & $\mathrm{relu}$ & $0$\\ 
 3e & $10$ & $4$ & $1000$ &  $1 \times 10^{-4}$ & $\mathrm{relu}$ & $5 \times 10^{-4}$\\ 
 4e & $30$ & $4$ & $1000$ &  $1 \times 10^{-4}$ & $\mathrm{relu}$ & $1 \times 10^{-4}$\\ 
\hline
\end{tabular}
\label{1dEuler_params}
\end{center}

\begin{figure}\label{1dEuler_sol}
\centering
\begin{subfigure}{.33\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{1dEulerEq/U.pdf}
\caption{}
\end{subfigure}%
\begin{subfigure}{.33\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{1dEulerEq/rho.pdf}
\caption{}
\end{subfigure}%
\begin{subfigure}{.33\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{1dEulerEq/E.pdf}
\caption{}
\end{subfigure}
\caption{Numerical solution of the contact discontinuity problem 1D Euler's equation using ENN at $t = 0.1$. (a): the solution velocity $u$. (b): the solution density $\rho$ (c): the total energy $E$. \mycircle{black!50!gray} \mycircle{black!40!gray} \mycircle{black!40!gray}: true solution.  \dotted \,: case 1e, \dashed \,: case 2e, \fullblack \,case 3e . \chainblack \,: case 4e}
\label{1dEuler_sol}
\end{figure}



\begin{figure}\label{1dEuler_xt}
\centering
\begin{subfigure}{.33\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{1dEulerEq/xtUTruth.pdf}
\caption{}
\end{subfigure}%
\begin{subfigure}{.33\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{1dEulerEq/xtrhoTruth.pdf}
\caption{}
\end{subfigure}%
\begin{subfigure}{.33\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{1dEulerEq/xtETruth.pdf}
\caption{}
\end{subfigure}
\centering
\begin{subfigure}{.33\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{1dEulerEq/xtUENN.pdf}
\caption{}
\end{subfigure}%
\begin{subfigure}{.33\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{1dEulerEq/xtrhoENN.pdf}
\caption{}
\end{subfigure}%
\begin{subfigure}{.33\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{1dEulerEq/xtEENN.pdf}
\caption{}
\end{subfigure}
\caption{Time history of numerical solution of the contact discontinuity problem 1D Euler's equation using ENN . (a) (b) (c): analytical solution. (d) (e) (f): solution from ENN}
\label{1dEuler_xt}
\end{figure}

